A Fokker-Planck Study of Dense Rotating Stellar Clusters

The dynamical evolution of dense stellar systems is simulated using a two-dimensional Fokker-Planck method, with the goal of providing a model for the formation of supermassive stars which could serve as seed objects for the supermassive black holes of quasars. This work follows and expands on earlier 1-D studies of spherical clusters of main-sequence stars. The 2-D approach allows for the study of rotating systems, as would be expected due to cosmological tidal torquing; other physical effects included are collisional mergers of stars and a bulk stellar bar perturbation in the gravitational potential. The 3 Myr main-sequence lifetime for large stars provides an upper limit on simulation times. Two general classes of initial systems are studied: Plummer spheres, which represent stellar clusters, and \gamma=0 spheres, which model galactic spheroids. At the initial densities of the modeled systems, mass segregation and runaway stellar collisions alone are insufficient to induce core collapse within the lifetime limit if no bar perturbation is included. However, core collapse is not a requirement for the formation of a massive object: the choice of stellar initial mass function is found to play a crucial role. When using an IMF similar to that observed for dense stellar clusters the simulations show that the stellar system forms massive (250M_\odot) objects by collisional mergers; in almost all such cases the presence of a stellar bar allows for sufficient additional outward transport of angular momentum that a core-collapse state is reached with corresponding further increase in the rate of formation of massive objects. In contrast, simulations using an IMF similar to that observed for field stars in general (which is weighted more towards lower masses) produce no massive objects, and reach core collapse only for initial models which represent the highest-density galactic spheriods.

==> OldStuff.tex <==
%used to be in Results.tex

\markup{The remaining subsections that were previously listed here were all old
thinking regarding pre-setaj0 runs of 1-, 2- and 3-mass systems that probably
aren't valid and (mostly) aren't scientifically interesting.  (The SMS run
might be interesting though; redo?).}

\begin{comment}
\section{OLD STUFF}

\section{Single-Mass Clusters}

\subsection{Non-rotating}
\markup{harold:prod/e4b/1mass/stdnlm9, currently to 35 (nm2=60 trying bigdt)}

\subsection{Rotating}
\markup{harold:prod/e4b/1mass/stdrot0nlm9, currently to 29; stdrot0nlm2 to 39}

\subsection{Rotating, with bar}
\markup{harold:1mass/stdbar60 to 67!}

\subsection{With Massive Stars}
\markup{ice:1mass5bar2/bigdt done; harold:1mass5 to 24, 1mass5rot/bigdt still going} 

\subsection{With Supermassive Stars}
\markup{zeus:prod/e4b/1mass50 \& 1mass50rot still going; trogdor~/prod/e4b/1mass50bar2}

\section{Two- and Three-Mass Clusters}\label{sect_2M}
\subsection{Non-rotating}
\markup{cfa0:2mass/40x40/nlm9 killed: badly unstable. try nm2=60? (only really needed if rot case also bad)}

\markup{harold:3massMS/40x40/bigdt to 17; nm2=60 retrying w/ big dt}

\subsection{Rotating}
\markup{harold:prod/e4b/2mass/40x40/nlm9/rot, but only to 20.  trying nm2=60}

\markup{harold:3massMS/40x40/stdrot gave endpts problem, both nm2=50 \& 60}

\subsection{Rotating, with bar}
\markup{ice:2mass/40x40/nlm2/stdbar up to 32}

\subsection{With Stellar Mergers}
\markup{cf: 2mass/rot ended early (at 11); nonrot not even bothered with.
trying rot w/ nm2=60}

\markup{harold:3massMS/40x40/bigdt/mrj only to 16.  nm2=60 worse.}

\markup{could also put 34x34 that shows 2mass v 3mass merger effect}

\subsection{With Massive Stars}
\markup{harold:2mass5 just started, with nm2=50 (60 was bad\bf NEEDED BIG DT?)}

\markup{harold:prod/e4b/2mass5rot9/bigdt basically just started}

\markup{ice:2mass5bar2  went way long.}

\section{Multi-Mass Clusters}\label{sect_multiM}

\subsection{Non-rotating}
\markup{cfa0:prod/e4b/9Kn9 only to 14.  cfa0:mrj only to 7.}

\markup{harold:prod/e4b/10Kn9/middt/restart12/ to 29, mrj4 failed.}

\subsection{Rotating}
\markup{harold:prod/e4b/9Kn9/rot only to 19, harold:mrj4 only to 17.}

\markup{harold:prod/e4b/10Kn9/middt/rot to 22, harold:mrj4 too.}

\subsection{Rotating, with bar}

\markup{cfa0~/prod/e4b/9Kn2/bar7/bigdt to 60! trog:mrj only to 25 though}

\markup{cfa0~/prod/e4b/10Kn2/bar7/bigdt to 48! cfa0:mrj too! (but no help)}
\end{comment}

